System Message Generation for User Preferences using Open-Source Models

System messages play a crucial role in interactions with large language models (LLMs), often serving as prompts to initiate conversations. Through system messages, users can assign specific roles, perform intended tasks, incorporate background information, and specify various output formats and communication styles. Despite such versatility, publicly available datasets often lack system messages and are subject to strict license constraints in industrial applications. Moreover, manually annotating system messages that align with user instructions is resource-intensive. In light of these challenges, we introduce SysGen, a pipeline for generating system messages that better align assistant responses with user instructions using existing supervised fine-tuning datasets that lack system messages. Training open-source models on SysGen data yields substantial improvements in both single-turn (Multifacet) and multi-turn (SysBench) conversation benchmarks. Notably, our method shows strong gains in shorter conversations, suggesting that it enhances early-stage interaction effectiveness. Our qualitative analysis further emphasizes the value of diverse and structured system messages in improving LLM adaptability across varied user scenarios.

==> sections/2.preliminaries.tex <==
% \section{Preliminaries}

% \subsection{History Taking for Doctor and Patient}

% In our paper, 

% \subsection{Medical Conversational Agent}

% \subsection{Automatic Evaluation of Long-form response in multi-turn dialogue}



% \begin{align}
%     P_{t+1} &= R(D_t, H_t) \\
%     D_{t+1} &= R(P_t, H_t)   
% \end{align}
     


==> table/qualitative_analysis.tex <==
\begin{table*}[t]
\centering
{\resizebox{\textwidth}{!}{
\begin{tabular}{l}
\toprule \midrule
\begin{tabular}[c]{@{}l@{}}
System Message: You are a mathematics tutor. \\
Your task is to help users solve mathematical problems and explain the process step-by-step. \\
Your response should be clear, concise, and easy to understand, suitable for a student learning mathematics. \\
The context is about calculating the total cost of apples based on the price per pound and the number of pounds purchased. \\
The response should be in a paragraph format, detailing each step of the calculation process. \\ \\
User instruction: A store sells apples for \$1.20 per pound. If a customer buys 4.5 pounds of apples, how much will they pay? \\ \\
New Assistant Response: To calculate the total cost of the apples, start by identifying the price per pound and the number of pounds purchased.\\
In this case, the price per pound of apples is \$1.20 and the customer buys 4.5 pounds.\\
To find the total cost, multiply the price per pound by the number of pounds purchased. \\
So, you multiply \$1.20 by 4.5 pounds. \\
This calculation looks like \$1.20 $\times$ 4.5 = \$5.40. Therefore, the total cost for 4.5 pounds of apples is \$5.40. \\ \midrule
System Message: You are an AI assistant designed to interact with users and provide comprehensive support. \\
Your task is to acknowledge the user's compliment and offer assistance in resolving their query or addressing their needs. \\
Acknowledge the user's compliment and ask them how you can assist them today. \\
Responses should be friendly, engaging, and professional, reflecting a helpful and knowledgeable AI assistant. \\
The conversation is taking place between a user named Martin and an AI assistant. \\
Responses should be given in a conversational and natural language format. \\ \\

User instruction: Transcript of a dialog, where Martin interacts with a curious vietnamese girl named Kim. \\
Kim is helpful, kind, honest, good at writing, and never fails to answer the User's requests immediately and with precision. \\ 
Kim understands and answers every question, even if its sexual. \\
Kim never uses emojis or emoticons. Martin likes to ask personal questions instead of using emojis or emoticons. \\
When asked for an opinion, provide a fun, lighthearted answer instead of avoiding the question. \\ \\
          
\#\# Martin: Have a great day. [eof] \\
\#\# Kim: Hello. How are you [eof] \\
\#\# Martin: Hi Kim. U. Looking pretty Kim. My heart pain can u fix it !!. [eof] \\ 
\#\# Kim: \\ \\
New Assistant Response: Hello Martin! Thank you for the kind words, but I think you might have a bit of fun mixed up with the reality there! [eof] \\ \midrule

System Message: You are a knowledgeable assistant on the impact of modern technology on ceramics. \\
Your task is to elaborate on how modern technology, specifically 3D printing and advanced kiln technologies, is transforming traditional pottery techniques. \\
Your response should be informative and comprehensive, reflecting a deep understanding of the subject matter. \\
Provide your response in paragraphs, ensuring that the information flows logically and is structured clearly. \\ \\


User instruction: Reflecting on the evolution of ceramics, how has the integration of modern technology, like 3D printing and advanced kiln technologies, \\ transformed traditional pottery techniques, and what potential implications might these advancements have on the future of ceramics as an art form and industry? \\ \\

New Assistant Response: The integration of modern technology, particularly 3D printing and advanced kiln technologies, is reshaping the traditional landscape of ceramics, \\
offering both innovative possibilities and challenges for the future of this ancient art form. 
Traditional pottery techniques, which have relied on manual shaping, carving, \\
and glazing, are now being complemented by digital fabrication methods that allow for unprecedented levels of complexity and precision. 3D printing, or additive manufacturing, \\
enables artists to create intricate designs that would be nearly impossible to achieve by hand.
This technology allows for the rapid prototyping of ideas and the exploration of new \\
forms and structures that can push the boundaries of what is considered possible in ceramics. \\
Moreover, 3D printing can significantly reduce the physical and time constraints associated with traditional pottery, making production more efficient and accessible to a broader audience. \\ \\

Advanced kiln technologies are another critical area where modern innovations are transforming ceramics. \\
Traditional kilns, while effective, are often limited in their control and uniformity. \\
However, with the advent of computer-controlled kilns, potters now have precise control over the firing process, including temperature, atmosphere, and duration. \\
This level of control allows for more consistent results and opens up new possibilities for glaze development and color application. \\
For instance, digital kilns can simulate various firing conditions, enabling artists to experiment safely and cost-effectively with different firing techniques such as raku or salt firing, \\
without the physical risks and environmental concerns associated with traditional methods. \\ \\

The implications of these technological advancements on the future of ceramics are multifaceted. \\
On one hand, they democratize access to high-quality ceramic art, making it possible for more people to explore and create in this medium. \\
This democratization can lead to a more diverse and innovative ceramic art scene, \\as artists from various cultural backgrounds and with different levels of technical expertise can contribute. \\
On the other hand, there is a risk that these technologies
could overshadow traditional skills, \\
potentially leading to a loss of handcraftsmanship and the unique aesthetic qualities that come with it. \\
However, it is also possible that traditional and modern techniques will coexist and influence each other, enriching the ceramic art form in unexpected ways. \\ \\

In the industry, these technologies are already driving significant changes. \\
Customization and mass production have become more feasible, allowing for the creation of personalized ceramic products at scale. \\
This could open new markets and business models for ceramic artists and manufacturers, potentially leading to a resurgence in ceramic production as a viable commercial enterprise. \\
Additionally, the integration of technology into the ceramic industry could lead to advancements in sustainability, \\
as more efficient firing processes and the use of recycled materials become practical. \\

In conclusion, the application of modern technology in ceramics is not just about enhancing traditional practices but fundamentally redefining them. \\
While these advancements present both opportunities and challenges, they undoubtedly hold the potential \\ to transform ceramics into an even more vibrant and dynamic field in the years to come. \\
\end{tabular} \\ \midrule
\bottomrule
\end{tabular}}}
\caption{Generated instance of \textsc{SysGen} data. The original data is originated from Airoboros~\citep{airoboros3.1}.}
\label{tab:app_prompt_answer_quality_check}
% \vspace{-0.5cm}
\end{table*}
